Topological properties of cellular automata on trees

We prove that there do not exist positively expansive cellular automata defined on the full k-ary tree shift (for k>=2). Moreover, we investigate some topological properties of these automata and their relationships, namely permutivity, surjectivity, preinjectivity, right-closingness and openness.

==> eptcsdata.tex <==
\providecommand{\firstpage}{255}
\providecommand{\publicationstatus}{E. Formenti (Ed.): AUTOMATA and JAC 2012 conferences\\
EPTCS 90, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.90.20}{10.4204/EPTCS.90.20}}

